Finding lensed direct-collapse black holes and supermassive primordial stars

Direct-collapse black holes (DCBHs) may be the seeds of the first quasars, over 200 of which have now been detected at $z > 6$ . The James Webb Space Telescope (JWST) could detect DCBHs in the near infrared (NIR) at $z \lesssim 20$ and probe the evolution of primordial quasars at their earliest stages, but only in narrow fields that may not capture many of them. Wide-field NIR surveys by Euclid and the Nancy Grace Roman Survey Telescope (RST) would enclose far greater numbers of DCBHs but only directly detect them at $z \lesssim 6 - 8$ because of their lower sensitivities. However, their large survey areas will cover thousands of galaxy clusters and massive galaxies that could gravitationally lense flux from DCBHs, boosting them above current Euclid and RST detection limits and revealing more of them than could otherwise be detected. Here, we estimate the minimum number density of strongly lensed DCBHs and supermassive primordial stars required for detection in surveys by Euclid, RST and JWST at $z \lesssim 20$. We find that for reasonable estimates of host halo numbers RST, Euclid, and JWST could potentially find hundreds of strongly-lensed DCBHs at $z = 7 - 20$. RST would detect the most objects at $z \lesssim 10$ and JWST would find the most at higher redshifts. Lensed supermassive primordial stars could potentially also be found, but in fewer numbers because of their short lifetimes.

==> pastedbib.tex <==
\begin{thebibliography}{50}
\expandafter\ifx\csname natexlab\endcsname\relax\def\natexlab#1{#1}\fi

\bibitem[{{Agarwal} {et~al.}(2016){Agarwal}, {Smith}, {Glover}, {Natarajan}, \&
  {Khochfar}}]{agarw15}
{Agarwal}, B., {Smith}, B., {Glover}, S., {Natarajan}, P., \& {Khochfar}, S.
  2016, \mnras, 459, 4209

\bibitem[{{Akeson} {et~al.}(2019){Akeson}, {Armus}, {Bachelet}, {Bailey},
  {Bartusek}, {Bellini}, {Benford}, {Bennett}, {Bhattacharya}, {Bohlin},
  {Boyer}, {Bozza}, {Bryden}, {Calchi Novati}, {Carpenter}, {Casertano},
  {Choi}, {Content}, {Dayal}, {Dressler}, {Dor{\'e}}, {Fall}, {Fan}, {Fang},
  {Filippenko}, {Finkelstein}, {Foley}, {Furlanetto}, {Kalirai}, {Gaudi},
  {Gilbert}, {Girard}, {Grady}, {Greene}, {Guhathakurta}, {Heinrich},
  {Hemmati}, {Hendel}, {Henderson}, {Henning}, {Hirata}, {Ho}, {Huff},
  {Hutter}, {Jansen}, {Jha}, {Johnson}, {Jones}, {Kasdin}, {Kelly}, {Kirshner},
  {Koekemoer}, {Kruk}, {Lewis}, {Macintosh}, {Madau}, {Malhotra}, {Mandel},
  {Massara}, {Masters}, {McEnery}, {McQuinn}, {Melchior}, {Melton},
  {Mennesson}, {Peeples}, {Penny}, {Perlmutter}, {Pisani}, {Plazas}, {Poleski},
  {Postman}, {Ranc}, {Rauscher}, {Rest}, {Roberge}, {Robertson}, {Rodney},
  {Rhoads}, {Rhodes}, {Ryan}, {Sahu}, {Sand}, {Scolnic}, {Seth}, {Shvartzvald},
  {Siellez}, {Smith}, {Spergel}, {Stassun}, {Street}, {Strolger}, {Szalay},
  {Trauger}, {Troxel}, {Turnbull}, {van der Marel}, {von der Linden}, {Wang},
  {Weinberg}, {Williams}, {Windhorst}, {Wollack}, {Wu}, {Yee}, \&
  {Zimmerman}}]{2019Akeson}
{Akeson}, R., {et~al.} 2019, arXiv e-prints, arXiv:1902.05569

\bibitem[{{Ba{\~n}ados} {et~al.}(2018){Ba{\~n}ados}, {Venemans},
  {Mazzucchelli}, {Farina}, {Walter}, {Wang}, {Decarli}, {Stern}, {Fan},
  {Davies}, {Hennawi}, {Simcoe}, {Turner}, {Rix}, {Yang}, {Kelson}, {Rudie}, \&
  {Winters}}]{ban18}
{Ba{\~n}ados}, E., {et~al.} 2018, \nat, 553, 473

\bibitem[{{Barrow} {et~al.}(2018){Barrow}, {Aykutalp}, \& {Wise}}]{bar18}
{Barrow}, K. S.~S., {Aykutalp}, A., \& {Wise}, J.~H. 2018, Nature Astronomy, 2,
  987

\bibitem[{{Baugh} {et~al.}(2005){Baugh}, {Lacey}, {Frenk}, {Granato}, {Silva},
  {Bressan}, {Benson}, \& {Cole}}]{2005Baugh}
{Baugh}, C.~M., {Lacey}, C.~G., {Frenk}, C.~S., {Granato}, G.~L., {Silva}, L.,
  {Bressan}, A., {Benson}, A.~J., \& {Cole}, S. 2005, \mnras, 356, 1191

\bibitem[{{Bradley} {et~al.}(2014){Bradley}, {Zitrin}, {Coe}, {Bouwens},
  {Postman}, {Balestra}, {Grillo}, {Monna}, {Rosati}, {Seitz}, {Host}, {Lemze},
  {Moustakas}, {Moustakas}, {Shu}, {Zheng}, {Broadhurst}, \& {et al.}}]{brd14}
{Bradley}, L.~D., {et~al.} 2014, ApJ, 792, 76

\bibitem[{{Di Matteo} {et~al.}(2012){Di Matteo}, {Khandai}, {DeGraf}, {Feng},
  {Croft}, {Lopez}, \& {Springel}}]{dm12}
{Di Matteo}, T., {Khandai}, N., {DeGraf}, C., {Feng}, Y., {Croft}, R.~A.~C.,
  {Lopez}, J., \& {Springel}, V. 2012, \apjl, 745, L29

\bibitem[{{Habouzit} {et~al.}(2016){Habouzit}, {Volonteri}, {Latif}, {Dubois},
  \& {Peirani}}]{hab16}
{Habouzit}, M., {Volonteri}, M., {Latif}, M., {Dubois}, Y., \& {Peirani}, S.
  2016, \mnras, 463, 529

\bibitem[{{Haemmerl{\'e}} {et~al.}(2018{\natexlab{a}}){Haemmerl{\'e}}, {Woods},
  {Klessen}, {Heger}, \& {Whalen}}]{hle18a}
{Haemmerl{\'e}}, L., {Woods}, T.~E., {Klessen}, R.~S., {Heger}, A., \&
  {Whalen}, D.~J. 2018{\natexlab{a}}, \apjl, 853, L3

\bibitem[{{Haemmerl{\'e}} {et~al.}(2018{\natexlab{b}}){Haemmerl{\'e}}, {Woods},
  {Klessen}, {Heger}, \& {Whalen}}]{hle18b}
---. 2018{\natexlab{b}}, \mnras, 474, 2757

\bibitem[{{Hartwig} {et~al.}(2018){Hartwig}, {Agarwal}, \& {Regan}}]{til18a}
{Hartwig}, T., {Agarwal}, B., \& {Regan}, J.~A. 2018, \mnras, 479, L23

\bibitem[{{Herrington} {et~al.}(2021){Herrington}, {Whalen}, \&
  {Wood}}]{herr21a}
{Herrington}, N., {Whalen}, D.~J., \& {Wood}, T.~E. 2021, \mnras, in prep

\bibitem[{{Hirano} {et~al.}(2017){Hirano}, {Hosokawa}, {Yoshida}, \&
  {Kuiper}}]{hir17}
{Hirano}, S., {Hosokawa}, T., {Yoshida}, N., \& {Kuiper}, R. 2017, Science,
  357, 1375

\bibitem[{{Hosokawa} {et~al.}(2013){Hosokawa}, {Yorke}, {Inayoshi}, {Omukai},
  \& {Yoshida}}]{hos13}
{Hosokawa}, T., {Yorke}, H.~W., {Inayoshi}, K., {Omukai}, K., \& {Yoshida}, N.
  2013, \apj, 778, 178

\bibitem[{{Johnson} {et~al.}(2013){Johnson}, {Whalen}, {Li}, \& {Holz}}]{jet13}
{Johnson}, J.~L., {Whalen}, D.~J., {Li}, H., \& {Holz}, D.~E. 2013, \apj, 771,
  116

\bibitem[{{Latif} {et~al.}(2015){Latif}, {Bovino}, {Grassi}, {Schleicher}, \&
  {Spaans}}]{latif15a}
{Latif}, M.~A., {Bovino}, S., {Grassi}, T., {Schleicher}, D.~R.~G., \&
  {Spaans}, M. 2015, \mnras, 446, 3163

\bibitem[{{Latif} \& {Khochfar}(2020)}]{latif20b}
{Latif}, M.~A., \& {Khochfar}, S. 2020, \mnras, 497, 3761

\bibitem[{{Latif} {et~al.}(2020){Latif}, {Khochfar}, \& {Whalen}}]{latif20a}
{Latif}, M.~A., {Khochfar}, S., \& {Whalen}, D. 2020, \apjl, 892, L4

\bibitem[{{Latif} {et~al.}(2022){Latif}, {Whalen}, {Khochfar}, {Herrington}, \&
  {Woods}}]{latif22b}
{Latif}, M.~A., {Whalen}, D.~J., {Khochfar}, S., {Herrington}, N.~P., \&
  {Woods}, T.~E. 2022, \nat, accepted

\bibitem[{{Laureijs} {et~al.}(2011){Laureijs}, {Amiaux}, {Arduini},
  {Augu{\`e}res}, {Brinchmann}, {Cole}, {Cropper}, {Dabin}, {Duvet}, {Ealet},
  \& et~al.}]{euclid}
{Laureijs}, R., {et~al.} 2011, arXiv:1110.3193

\bibitem[{{Li} {et~al.}(2007){Li}, {Hernquist}, {Robertson}, {Cox}, {Hopkins},
  {Springel}, {Gao}, {Di Matteo}, {Zentner}, {Jenkins}, \& {Yoshida}}]{li07}
{Li}, Y., {et~al.} 2007, \apj, 665, 187

\bibitem[{{Meneghetti} {et~al.}(2020){Meneghetti}, {Davoli}, {Bergamini},
  {Rosati}, {Natarajan}, {Giocoli}, {Caminha}, {Metcalf}, {Rasia}, {Borgani},
  {Calura}, {Grillo}, {Mercurio}, \& {Vanzella}}]{2020Meneghetti}
{Meneghetti}, M., {et~al.} 2020, Science, 369, 1347

\bibitem[{{Mortlock} {et~al.}(2011){Mortlock}, {Warren}, {Venemans}, {Patel},
  {Hewett}, {McMahon}, {Simpson}, {Theuns}, {Gonz{\'a}les-Solares}, {Adamson},
  {Dye}, {Hambly}, {Hirst}, {Irwin}, {Kuiper}, {Lawrence}, \&
  {R{\"o}ttgering}}]{mort11}
{Mortlock}, D.~J., {et~al.} 2011, \nat, 474, 616

\bibitem[{{Natarajan} {et~al.}(2017){Natarajan}, {Pacucci}, {Ferrara},
  {Agarwal}, {Ricarte}, {Zackrisson}, \& {Cappelluti}}]{nat17}
{Natarajan}, P., {Pacucci}, F., {Ferrara}, A., {Agarwal}, B., {Ricarte}, A.,
  {Zackrisson}, E., \& {Cappelluti}, N. 2017, \apj, 838, 117

\bibitem[{{Pacucci} {et~al.}(2016){Pacucci}, {Ferrara}, {Grazian}, {Fiore},
  {Giallongo}, \& {Puccetti}}]{2016Pacucci}
{Pacucci}, F., {Ferrara}, A., {Grazian}, A., {Fiore}, F., {Giallongo}, E., \&
  {Puccetti}, S. 2016, \mnras, 459, 1432

\bibitem[{{Pacucci} {et~al.}(2015){Pacucci}, {Ferrara}, {Volonteri}, \&
  {Dubus}}]{pac15}
{Pacucci}, F., {Ferrara}, A., {Volonteri}, M., \& {Dubus}, G. 2015, \mnras,
  454, 3771

\bibitem[{{Patrick} {et~al.}(2020){Patrick}, {Whalen}, {Elford}, \&
  {Latif}}]{pat21a}
{Patrick}, S.~J., {Whalen}, D.~J., {Elford}, J.~S., \& {Latif}, M.~A. 2020,
  arXiv e-prints, arXiv:2012.11612

\bibitem[{{Regan} \& {Downes}(2018)}]{rd18}
{Regan}, J.~A., \& {Downes}, T.~P. 2018, \mnras, 475, 4636

\bibitem[{{Rieke} {et~al.}(2019){Rieke}, {Arribas}, {Bunker}, {Charlot},
  {Finkelstein}, {Maiolino}, {Robertson}, {Willott}, {Windhorst}, {Eisenstein},
  {Nelson}, {Tacchella}, {Egami}, {Endsley}, {Frye}, {Hainline}, {Hviding},
  {Rieke}, {Williams}, {Willmer}, \& {Woodrum}}]{riek19}
{Rieke}, M., {et~al.} 2019, \baas, 51, 45

\bibitem[{{Salmon} {et~al.}(2020){Salmon}, {Coe}, {Bradley}, {Bouwens},
  {Brada{\v{c}}}, {Huang}, {Oesch}, {Stark}, {Sharon}, {Trenti}, {Avila},
  {Ogaz}, {Andrade-Santos}, {Carrasco}, {Cerny}, {Dawson}, {Frye}, {Hoag},
  {Johnson}, {Jones}, {Lam}, {Lovisari}, {Mainali}, {Past}, {Paterno-Mahler},
  {Peterson}, {Riess}, {Rodney}, {Ryan}, {Sendra-Server}, {Strait}, {Strolger},
  {Umetsu}, {Vulcani}, \& {Zitrin}}]{2020Salmon}
{Salmon}, B., {et~al.} 2020, \apj, 889, 189

\bibitem[{{Salpeter}(1964)}]{sal64}
{Salpeter}, E.~E. 1964, \apj, 140, 796

\bibitem[{{Smidt} {et~al.}(2018){Smidt}, {Whalen}, {Johnson}, {Surace}, \&
  {Li}}]{smidt18}
{Smidt}, J., {Whalen}, D.~J., {Johnson}, J.~L., {Surace}, M., \& {Li}, H. 2018,
  \apj, 865, 126

\bibitem[{{Smith} {et~al.}(2018){Smith}, {Regan}, {Downes}, {Norman}, {O'Shea},
  \& {Wise}}]{srd18}
{Smith}, B.~D., {Regan}, J.~A., {Downes}, T.~P., {Norman}, M.~L., {O'Shea},
  B.~W., \& {Wise}, J.~H. 2018, \mnras, 480, 3762

\bibitem[{{Surace} {et~al.}(2019){Surace}, {Zackrisson}, {Whalen}, {Hartwig},
  {Glover}, {Woods}, {Heger}, \& {Glover}}]{sur19a}
{Surace}, M., {Zackrisson}, E., {Whalen}, D.~J., {Hartwig}, T., {Glover},
  S.~C.~O., {Woods}, T.~E., {Heger}, A., \& {Glover}, S.~C.~O. 2019, \mnras,
  488, 3995

\bibitem[{{Surace} {et~al.}(2018){Surace}, {Whalen}, {Hartwig}, {Zackrisson},
  {Glover}, {Patrick}, {Woods}, {Heger}, \& {Haemmerl{\'e}}}]{sur18a}
{Surace}, M., {et~al.} 2018, \apjl, 869, L39

\bibitem[{{Valentini} {et~al.}(2021){Valentini}, {Gallerani}, \&
  {Ferrara}}]{vgf21}
{Valentini}, M., {Gallerani}, S., \& {Ferrara}, A. 2021, \mnras, 507, 1

\bibitem[{{Valiante} {et~al.}(2017){Valiante}, {Agarwal}, {Habouzit}, \&
  {Pezzulli}}]{rosa17}
{Valiante}, R., {Agarwal}, B., {Habouzit}, M., \& {Pezzulli}, E. 2017, \pasa,
  34, e031

\bibitem[{{Vanzella} {et~al.}(2014){Vanzella}, {Fontana}, {Zitrin}, {Coe},
  {Bradley}, {Postman}, {Grazian}, {Castellano}, {Pentericci}, {Giavalisco},
  {Rosati}, {Nonino}, {Smit}, {Balestra}, {Bouwens}, {Cristiani}, \& {et
  al.}}]{vanz14}
{Vanzella}, E., {et~al.} 2014, ApJL, 783, L12

\bibitem[{{Vikaeus} {et~al.}(2022){Vikaeus}, {Zackrisson}, {Schaerer},
  {Visbal}, {Fransson}, {Malhotra}, {Rhoads}, \& {Sahl{\'e}n}}]{vik21a}
{Vikaeus}, A., {Zackrisson}, E., {Schaerer}, D., {Visbal}, E., {Fransson}, E.,
  {Malhotra}, S., {Rhoads}, J., \& {Sahl{\'e}n}, M. 2022, \mnras

\bibitem[{{Wang} {et~al.}(2021){Wang}, {Yang}, {Fan}, {Hennawi}, {Barth},
  {Banados}, {Bian}, {Boutsia}, {Connor}, {Davies}, {Decarli}, {Eilers},
  {Farina}, {Green}, {Jiang}, {Li}, {Mazzucchelli}, {Nanni}, {Schindler},
  {Venemans}, {Walter}, {Wu}, \& {Yue}}]{wang21}
{Wang}, F., {et~al.} 2021, \apjl, 907, L1

\bibitem[{{Welch} {et~al.}(2022){Welch}, {Coe}, {Diego}, {Zitrin},
  {Zackrisson}, {Dimauro}, {Jiménez-Teja}, {Kelly}, {Mahler}, {Oguri},
  {Timmes}, {Windhorst}, {Florian}, {de Mink}, {Avila}, {Anderson}, {Bradley},
  {Sharon}, {Vikaeus}, {McCandliss}, {Brada{\v{c}}}, {Rigby}, {Frye}, {Toft},
  {Strait}, {Trenti}, {Sharma}, {Andrade-Santos}, \& {Broadhurst}}]{2022Welch}
{Welch}, B., {et~al.} 2022, Nature, 603, 815

\bibitem[{{Whalen} {et~al.}(2004){Whalen}, {Abel}, \& {Norman}}]{wan04}
{Whalen}, D., {Abel}, T., \& {Norman}, M.~L. 2004, \apj, 610, 14

\bibitem[{{Whalen} \& {Fryer}(2012)}]{wf12}
{Whalen}, D.~J., \& {Fryer}, C.~L. 2012, \apjl, 756, L19

\bibitem[{{Whalen} {et~al.}(2020{\natexlab{a}}){Whalen}, {Mezcua}, {Meiksin},
  {Hartwig}, \& {Latif}}]{wet20a}
{Whalen}, D.~J., {Mezcua}, M., {Meiksin}, A., {Hartwig}, T., \& {Latif}, M.~A.
  2020{\natexlab{a}}, \apjl, 896, L45

\bibitem[{{Whalen} {et~al.}(2020{\natexlab{b}}){Whalen}, {Surace}, {Bernhardt},
  {Zackrisson}, {Pacucci}, {Ziegler}, \& {Hirschmann}}]{wet20b}
{Whalen}, D.~J., {Surace}, M., {Bernhardt}, C., {Zackrisson}, E., {Pacucci},
  F., {Ziegler}, B., \& {Hirschmann}, M. 2020{\natexlab{b}}, \apjl, 897, L16

\bibitem[{{Woods} {et~al.}(2017){Woods}, {Heger}, {Whalen}, {Haemmerl{\'e}}, \&
  {Klessen}}]{tyr17}
{Woods}, T.~E., {Heger}, A., {Whalen}, D.~J., {Haemmerl{\'e}}, L., \&
  {Klessen}, R.~S. 2017, \apjl, 842, L6

\bibitem[{{Woods} {et~al.}(2021){Woods}, {Patrick}, {Elford}, {Whalen}, \&
  {Heger}}]{tyr21a}
{Woods}, T.~E., {Patrick}, S., {Elford}, J.~S., {Whalen}, D.~J., \& {Heger}, A.
  2021, \apj, 915, 110

\bibitem[{{Woods} {et~al.}(2019){Woods}, {Agarwal}, {Bromm}, {Bunker}, {Chen},
  {Chon}, {Ferrara}, {Glover}, {Haemmerl{\'e}}, {Haiman}, {Hartwig}, {Heger},
  {Hirano}, {Hosokawa}, {Inayoshi}, {Klessen}, {Kobayashi}, {Koliopanos},
  {Latif}, {Li}, {Mayer}, {Mezcua}, {Natarajan}, {Pacucci}, {Rees}, {Regan},
  {Sakurai}, {Salvadori}, {Schneider}, {Surace}, {Tanaka}, {Whalen}, \&
  {Yoshida}}]{titans}
{Woods}, T.~E., {et~al.} 2019, Publications of the Astronomical Society of
  Australia, 36, e027

\bibitem[{{Zackrisson} {et~al.}(2015){Zackrisson}, {Gonz{\'a}lez}, {Eriksson},
  {Asadi}, {Safranek-Shrader}, {Trenti}, \& {Inoue}}]{zak15}
{Zackrisson}, E., {Gonz{\'a}lez}, J., {Eriksson}, S., {Asadi}, S.,
  {Safranek-Shrader}, C., {Trenti}, M., \& {Inoue}, A.~K. 2015, \mnras, 449,
  3057

\bibitem[{{Zhu} {et~al.}(2020){Zhu}, {Li}, {Li}, {Maji}, {Yajima}, {Schneider},
  \& {Hernquist}}]{zhu20}
{Zhu}, Q., {Li}, Y., {Li}, Y., {Maji}, M., {Yajima}, H., {Schneider}, R., \&
  {Hernquist}, L. 2020, arXiv e-prints, arXiv:2012.01458

\end{thebibliography}
